Randomized Value Functions via Posterior State-Abstraction Sampling

State abstraction has been an essential tool for dramatically improving the sample efficiency of reinforcement-learning algorithms. Indeed, by exposing and accentuating various types of latent structure within the environment, different classes of state abstraction have enabled improved theoretical guarantees and empirical performance. When dealing with state abstractions that capture structure in the value function, however, a standard assumption is that the true abstraction has been supplied or unrealistically computed a priori, leaving open the question of how to efficiently uncover such latent structure while jointly seeking out optimal behavior. Taking inspiration from the bandit literature, we propose that an agent seeking out latent task structure must explicitly represent and maintain its uncertainty over that structure as part of its overall uncertainty about the environment. We introduce a practical algorithm for doing this using two posterior distributions over state abstractions and abstract-state values. In empirically validating our approach, we find that substantial performance gains lie in the multi-task setting where tasks share a common, low-dimensional representation.

==> StateAbstractionMatrixFact(1)/algorithms/ps2_alg.tex <==
\begin{algorithm}[tbh]
\caption{Posterior State-Abstraction Sampling with Hypermodels \& Variance-IDS}
\label{alg:qmf}
\begin{algorithmic}
   \STATE {\bfseries Input:} Reference distributions $p_{z_\phi}, p_{z_\psi} = \mc{N}(0,I)$, Minibatch size $m$, Learning rate $\alpha$, Regularization parameters $\lambda$, Noise variances $\sigma^2_\phi$, $\sigma^2_\psi$
   \STATE Initialize $\mf{H}^\phi_\nu, \mf{H}^\psi_\nu$ 
   \STATE $\mc{D} \leftarrow \emptyset$
   \FOR{$t=1$ {\bfseries to} $T$}
   \FOR{$t=1$ {\bfseries to} $H$}
        \STATE Sample $Z = \{(z_\phi, z_\psi)_1, \ldots, (z_\phi, z_\psi)_K\}, z_\phi \sim p_{z_\phi}(\cdot), z_\psi \sim p_{z_\psi}(\cdot)$
        
        \STATE $\hat{Q}^\star_{(z_\phi,z_\psi)}(s,a) \triangleq \langle \mf{H}^\phi_\nu(z_\phi)(s),\mf{H}^\psi_\nu(z_\psi,\mf{H}^\phi_\nu(z_\phi))(a)\rangle$
        
        \STATE $\hat{\Delta}_a(s) \triangleq \frac{1}{|Z|} \sum\limits_{i=1}^K \max\limits_{a^\star \in \mc{A}} \hat{Q}^\star_{(z_\phi,z_\psi)_i}(s,a^\star) - \hat{Q}^\star_{(z_\phi,z_\psi)_i}(s,a)]$
    
        \STATE $\tilde{Z}(a) = \{(z_\phi,z_\psi) | (z_\phi,z_\psi) \in Z, a = \argmax\limits_{a^\star \in \mc{A}} \hat{Q}^\star_{(z_\phi,z_\psi)}(s,a^\star)\}$
        
        \STATE $\hat{v}_a(s) \triangleq \sum\limits_{a^\star \in \mc{A}} \frac{|\tilde{Z}(a^\star)|}{|Z|}(\frac{1}{|\tilde{Z}(a^\star)|} \sum\limits_{(z_\phi,z_\psi) \in \tilde{Z}(a^\star)} \hat{Q}^\star_{(z_\phi,z_\psi)}(s,a) - \frac{1}{|Z|} \sum\limits_{(z_\phi,z_\psi) \in Z} \hat{Q}^\star_{(z_\phi,z_\psi)}(s,a))^2$
    
        \STATE $\pi(\cdot | s_h) = \min\limits_{\pi \in \Delta(\mc{A})} \frac{\bE_{a \sim \pi}[(\hat{\Delta}_a(s))^2]}{\bE_{a \sim \pi}[\hat{v}_a(s)]}$
    
        \STATE Take action $a_h \sim \pi(\cdot|s_h)$ and observe $r_h, s_{h+1}$
    
        \STATE Sample random perturbations $\eta_\phi \sim \mc{N}(0, \sigma^2_\phi I), \eta_\psi \sim \mc{N}(0, \sigma^2_\psi I)$
    
        \STATE $\mc{D} \rightarrow \mc{D} \cup \{(s_h,a_h,r_h,s_{h+1},\eta_\phi, \eta_\psi)\}$
        
        \STATE Sample random minibatch $\tilde{\mc{D}} \stackrel{m}{\sim} \text{Uniform}(\mc{D})$
        
        % $\mc{R}(z_\phi, z_\psi, \nu) \triangleq \lambda||\mf{H}^\phi_\nu(z_\phi) - \mf{H}^\phi_{\nu_0}(z_\phi)||^2_2 + \lambda||\mf{H}^\psi_\nu(z_\psi, \mf{H}^\phi_\nu(z_\phi)) - \mf{H}^\psi_{\nu_0}(z_\psi, \mf{H}^\phi_{\nu_0}(z_\phi))||^2_2$
        
        % $\mc{L}(\nu,\tilde{\mc{D}}) = \bE_{\substack{z_\phi \sim p_z(\cdot) \\ z_\psi \sim p_z(\cdot)}}[\frac{1}{m} \sum\limits_{\tilde{\mc{D}}}(r + \max\limits_{a' \in \mc{A}}     \hat{Q}^\star_{z_\phi,z_\psi}(s',a') + \eta_\phi^Tz_\phi + \eta_\psi^Tz_\psi - \hat{Q}^\star_{z_\phi,z_\psi}(s,a))^2 +  \mc{R}(z_\phi, z_\psi, \nu)]$
        
        \STATE $\nu \leftarrow \nu - \alpha \nabla_\nu \mc{L}(\nu,\tilde{\mc{D}})$
   \ENDFOR
   \ENDFOR
\end{algorithmic}
\end{algorithm}


% \begin{algorithm}[H]
% \SetAlgoLined


% \For{t $1,\ldots,T$}{
%     \For{h $1,\ldots,H$}{
%         Sample $Z = \{(z_\phi, z_\psi)_1, \ldots, (z_\phi, z_\psi)_K\}, z_\phi \sim p_{z_\phi}(\cdot), z_\psi \sim p_{z_\psi}(\cdot)$
        
%         $\hat{Q}^\star_{(z_\phi,z_\psi)}(s,a) \triangleq \langle \mf{H}^\phi_\nu(z_\phi)(s),\mf{H}^\psi_\nu(z_\psi,\mf{H}^\phi_\nu(z_\phi))(a)\rangle$
        
%         $\hat{\Delta}_a(s) \triangleq \frac{1}{|Z|} \sum\limits_{i=1}^K \max\limits_{a^\star \in \mc{A}} \hat{Q}^\star_{(z_\phi,z_\psi)_i}(s,a^\star) - \hat{Q}^\star_{(z_\phi,z_\psi)_i}(s,a)]$
    
%         $\tilde{Z}(a) = \{(z_\phi,z_\psi) | (z_\phi,z_\psi) \in Z, a = \argmax\limits_{a^\star \in \mc{A}} \hat{Q}^\star_{(z_\phi,z_\psi)}(s,a^\star)\}$
        
%         $\hat{v}_a(s) \triangleq \sum\limits_{a^\star \in \mc{A}} \frac{|\tilde{Z}(a^\star)|}{|Z|}(\frac{1}{|\tilde{Z}(a^\star)|} \sum\limits_{(z_\phi,z_\psi) \in \tilde{Z}(a^\star)} \hat{Q}^\star_{(z_\phi,z_\psi)}(s,a) - \frac{1}{|Z|} \sum\limits_{(z_\phi,z_\psi) \in Z} \hat{Q}^\star_{(z_\phi,z_\psi)}(s,a))^2$
    
%         $\pi(\cdot | s_h) = \min\limits_{\pi \in \Delta(\mc{A})} \frac{\bE_{a \sim \pi}[(\hat{\Delta}_a(s))^2]}{\bE_{a \sim \pi}[\hat{v}_a(s)]}$
    
%         Take action $a_h \sim \pi(\cdot|s_h)$ and observe $r_h, s_{h+1}$
    
%         Sample random perturbations $\eta_\phi \sim \mc{N}(0, \sigma^2_\phi I), \eta_\psi \sim \mc{N}(0, \sigma^2_\psi I)$
    
%         $\mc{D} \rightarrow \mc{D} \cup \{(s_h,a_h,r_h,s_{h+1},\eta_\phi, \eta_\psi)\}$
        
%         Sample random minibatch $\tilde{\mc{D}} \stackrel{m}{\sim} \text{Uniform}(\mc{D})$
        
%         % $\mc{R}(z_\phi, z_\psi, \nu) \triangleq \lambda||\mf{H}^\phi_\nu(z_\phi) - \mf{H}^\phi_{\nu_0}(z_\phi)||^2_2 + \lambda||\mf{H}^\psi_\nu(z_\psi, \mf{H}^\phi_\nu(z_\phi)) - \mf{H}^\psi_{\nu_0}(z_\psi, \mf{H}^\phi_{\nu_0}(z_\phi))||^2_2$
        
%         % $\mc{L}(\nu,\tilde{\mc{D}}) = \bE_{\substack{z_\phi \sim p_z(\cdot) \\ z_\psi \sim p_z(\cdot)}}[\frac{1}{m} \sum\limits_{\tilde{\mc{D}}}(r + \max\limits_{a' \in \mc{A}}     \hat{Q}^\star_{z_\phi,z_\psi}(s',a') + \eta_\phi^Tz_\phi + \eta_\psi^Tz_\psi - \hat{Q}^\star_{z_\phi,z_\psi}(s,a))^2 +  \mc{R}(z_\phi, z_\psi, \nu)]$
        
%         $\nu \leftarrow \nu - \alpha \nabla_\nu \mc{L}(\nu,\tilde{\mc{D}})$
%     }
% }

% \end{algorithm}

==> StateAbstractionMatrixFact(1)/commands.tex <==
% Dynamically sized mid bar.
\newcommand{\bigmid}{\mathrel{\Big|}}

% ---- Colors and Notes ----
\definecolor{dblue}{RGB}{98, 140, 190}
\definecolor{dlblue}{RGB}{216, 235, 255}
\definecolor{dgreen}{RGB}{124, 155, 127}
\definecolor{dpink}{RGB}{207, 166, 208}
\definecolor{dyellow}{RGB}{255, 248, 199}
\definecolor{dgray}{RGB}{46, 49, 49}

% URL
\newcommand{\durl}[1]{\textcolor{dblue}{\underline{\url{#1}}}}

% Circled Numbers
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=0.7pt] (char) {\footnotesize{#1}};}}
% From: http://tex.stackexchange.com/questions/7032/good-way-to-make-textcircled-numbers

% Under set numbered subset of equation
\newcommand{\numeq}[3]{\underset{\textcolor{#2}{\circled{#1}}}{\textcolor{#2}{#3}}}

% ---- Abbreviations -----
\newcommand{\tc}[2]{\textcolor{#1}{#2}}
\newcommand{\ubr}[1]{\underbrace{#1}}
\newcommand{\uset}[2]{\underset{#1}{#2}}
\newcommand{\eps}{\varepsilon}

% Typical limit:
\newcommand{\nlim}{\underset{n \rightarrow \infty}{\lim}}
\newcommand{\nsum}{\sum_{i = 1}^n}
\newcommand{\nprod}{\prod_{i = 1}^n}

% Add an hrule with some space
\newcommand{\spacerule}{\begin{center}\hdashrule{2cm}{1pt}{1pt}\end{center}}

% Mathcal and Mathbb
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mf}[1]{\mathfrak{#1}}
\newcommand{\indic}{\mathbbm{1}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\rank}{\text{rank}}
\newcommand{\kl}[2]{D_{\text{KL}}(#1 || #2)}

\newcommand{\ra}{\rightarrow}
\newcommand{\la}{\leftarrow}

% argmin, argmax.
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% ---- Figures, Boxes, Theorems, Etc. ----

% Basic Image
\newcommand{\img}[2]{
\begin{center}
\includegraphics[scale=#2]{#1}
\end{center}}

% Put a fancy box around things.
\newcommand{\dbox}[1]{
\begin{mdframed}[roundcorner=4pt, backgroundcolor=gray!5]
\vspace{1mm}
{#1}
\end{mdframed}
}

%  --- PROOFS ---

% Inner environment for Proofs
\newmdenv[
  topline=false,
  bottomline=false,
  rightline = false,
  leftmargin=10pt,
  rightmargin=0pt,
  innertopmargin=0pt,
  innerbottommargin=0pt
]{innerproof}

% Proof Command
%\newenvironment{dproof}{\begin{proof} \text{\vspace{2mm}} \begin{innerproof}}{\end{innerproof}\end{proof}\vspace{4mm}}
\newenvironment{dproof}[1][Proof]{\begin{proof}[#1] \text{\vspace{2mm}} \begin{innerproof}}{\end{innerproof}\end{proof}\vspace{4mm}}


% Dave Definition
\newcounter{DaveDefCounter}
\setcounter{DaveDefCounter}{1}

\newcommand{\ddef}[2]
{
\begin{mdframed}[roundcorner=1pt, backgroundcolor=white]
\vspace{1mm}
{\bf Definition \theDaveDefCounter} (#1): {\it #2}
\stepcounter{DaveDefCounter}
\end{mdframed}
}

% Block Quote
\newenvironment{dblockquote}[2]{
\begin{blockquote}
#2
\vspace{-2mm}\hspace{10mm}{#1} \\
\end{blockquote}}

% Algorithm
\newenvironment{dalg}[1]
{\begin{algorithm}\caption{#1}\begin{algorithmic}}
{\end{algorithmic}\end{algorithm}}

% Dave Table
\newenvironment{dtable}[1]
{\begin{figure}[h]
\centering
\begin{tabular}{#1}\toprule}
{\bottomrule
\end{tabular}
\end{figure}}

% For numbering the last of an align*
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}



\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{example}{Example}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{question}{Question}

==> algorithms/ps2_alg.tex <==
\begin{algorithm}[tbh]
\caption{Posterior State-Abstraction Sampling with Hypermodels \& Variance-IDS}
\label{alg:qmf}
\begin{algorithmic}
   \STATE {\bfseries Input:} Reference distributions $p_{z_\phi}, p_{z_\psi} = \mc{N}(0,I)$, Minibatch size $m$, Learning rate $\alpha$, Regularization parameters $\lambda$, Noise variances $\sigma^2_\phi$, $\sigma^2_\psi$
   \STATE Initialize $\mf{H}^\phi_\nu, \mf{H}^\psi_\nu$ 
   \STATE $\mc{D} \leftarrow \emptyset$
   \FOR{$t=1$ {\bfseries to} $T$}
   \FOR{$t=1$ {\bfseries to} $H$}
        \STATE Sample $Z = \{(z_\phi, z_\psi)_1, \ldots, (z_\phi, z_\psi)_K\}, z_\phi \sim p_{z_\phi}(\cdot), z_\psi \sim p_{z_\psi}(\cdot)$
        
        \STATE $\hat{Q}^\star_{(z_\phi,z_\psi)}(s,a) \triangleq \langle \mf{H}^\phi_\nu(z_\phi)(s),\mf{H}^\psi_\nu(z_\psi,\mf{H}^\phi_\nu(z_\phi))(a)\rangle$
        
        \STATE $\hat{\Delta}_a(s) \triangleq \frac{1}{|Z|} \sum\limits_{i=1}^K \max\limits_{a^\star \in \mc{A}} \hat{Q}^\star_{(z_\phi,z_\psi)_i}(s,a^\star) - \hat{Q}^\star_{(z_\phi,z_\psi)_i}(s,a)]$
    
        \STATE $\tilde{Z}(a) = \{(z_\phi,z_\psi) | (z_\phi,z_\psi) \in Z, a = \argmax\limits_{a^\star \in \mc{A}} \hat{Q}^\star_{(z_\phi,z_\psi)}(s,a^\star)\}$
        
        \STATE $\hat{v}_a(s) \triangleq \sum\limits_{a^\star \in \mc{A}} \frac{|\tilde{Z}(a^\star)|}{|Z|}(\frac{1}{|\tilde{Z}(a^\star)|} \sum\limits_{(z_\phi,z_\psi) \in \tilde{Z}(a^\star)} \hat{Q}^\star_{(z_\phi,z_\psi)}(s,a) - \frac{1}{|Z|} \sum\limits_{(z_\phi,z_\psi) \in Z} \hat{Q}^\star_{(z_\phi,z_\psi)}(s,a))^2$
    
        \STATE $\pi(\cdot | s_h) = \min\limits_{\pi \in \Delta(\mc{A})} \frac{\bE_{a \sim \pi}[(\hat{\Delta}_a(s))^2]}{\bE_{a \sim \pi}[\hat{v}_a(s)]}$
    
        \STATE Take action $a_h \sim \pi(\cdot|s_h)$ and observe $r_h, s_{h+1}$
    
        \STATE Sample random perturbations $\eta_\phi \sim \mc{N}(0, \sigma^2_\phi I), \eta_\psi \sim \mc{N}(0, \sigma^2_\psi I)$
    
        \STATE $\mc{D} \rightarrow \mc{D} \cup \{(s_h,a_h,r_h,s_{h+1},\eta_\phi, \eta_\psi)\}$
        
        \STATE Sample random minibatch $\tilde{\mc{D}} \stackrel{m}{\sim} \text{Uniform}(\mc{D})$
        
        % $\mc{R}(z_\phi, z_\psi, \nu) \triangleq \lambda||\mf{H}^\phi_\nu(z_\phi) - \mf{H}^\phi_{\nu_0}(z_\phi)||^2_2 + \lambda||\mf{H}^\psi_\nu(z_\psi, \mf{H}^\phi_\nu(z_\phi)) - \mf{H}^\psi_{\nu_0}(z_\psi, \mf{H}^\phi_{\nu_0}(z_\phi))||^2_2$
        
        % $\mc{L}(\nu,\tilde{\mc{D}}) = \bE_{\substack{z_\phi \sim p_z(\cdot) \\ z_\psi \sim p_z(\cdot)}}[\frac{1}{m} \sum\limits_{\tilde{\mc{D}}}(r + \max\limits_{a' \in \mc{A}}     \hat{Q}^\star_{z_\phi,z_\psi}(s',a') + \eta_\phi^Tz_\phi + \eta_\psi^Tz_\psi - \hat{Q}^\star_{z_\phi,z_\psi}(s,a))^2 +  \mc{R}(z_\phi, z_\psi, \nu)]$
        
        \STATE $\nu \leftarrow \nu - \alpha \nabla_\nu \mc{L}(\nu,\tilde{\mc{D}})$
   \ENDFOR
   \ENDFOR
\end{algorithmic}
\end{algorithm}


% \begin{algorithm}[H]
% \SetAlgoLined


% \For{t $1,\ldots,T$}{
%     \For{h $1,\ldots,H$}{
%         Sample $Z = \{(z_\phi, z_\psi)_1, \ldots, (z_\phi, z_\psi)_K\}, z_\phi \sim p_{z_\phi}(\cdot), z_\psi \sim p_{z_\psi}(\cdot)$
        
%         $\hat{Q}^\star_{(z_\phi,z_\psi)}(s,a) \triangleq \langle \mf{H}^\phi_\nu(z_\phi)(s),\mf{H}^\psi_\nu(z_\psi,\mf{H}^\phi_\nu(z_\phi))(a)\rangle$
        
%         $\hat{\Delta}_a(s) \triangleq \frac{1}{|Z|} \sum\limits_{i=1}^K \max\limits_{a^\star \in \mc{A}} \hat{Q}^\star_{(z_\phi,z_\psi)_i}(s,a^\star) - \hat{Q}^\star_{(z_\phi,z_\psi)_i}(s,a)]$
    
%         $\tilde{Z}(a) = \{(z_\phi,z_\psi) | (z_\phi,z_\psi) \in Z, a = \argmax\limits_{a^\star \in \mc{A}} \hat{Q}^\star_{(z_\phi,z_\psi)}(s,a^\star)\}$
        
%         $\hat{v}_a(s) \triangleq \sum\limits_{a^\star \in \mc{A}} \frac{|\tilde{Z}(a^\star)|}{|Z|}(\frac{1}{|\tilde{Z}(a^\star)|} \sum\limits_{(z_\phi,z_\psi) \in \tilde{Z}(a^\star)} \hat{Q}^\star_{(z_\phi,z_\psi)}(s,a) - \frac{1}{|Z|} \sum\limits_{(z_\phi,z_\psi) \in Z} \hat{Q}^\star_{(z_\phi,z_\psi)}(s,a))^2$
    
%         $\pi(\cdot | s_h) = \min\limits_{\pi \in \Delta(\mc{A})} \frac{\bE_{a \sim \pi}[(\hat{\Delta}_a(s))^2]}{\bE_{a \sim \pi}[\hat{v}_a(s)]}$
    
%         Take action $a_h \sim \pi(\cdot|s_h)$ and observe $r_h, s_{h+1}$
    
%         Sample random perturbations $\eta_\phi \sim \mc{N}(0, \sigma^2_\phi I), \eta_\psi \sim \mc{N}(0, \sigma^2_\psi I)$
    
%         $\mc{D} \rightarrow \mc{D} \cup \{(s_h,a_h,r_h,s_{h+1},\eta_\phi, \eta_\psi)\}$
        
%         Sample random minibatch $\tilde{\mc{D}} \stackrel{m}{\sim} \text{Uniform}(\mc{D})$
        
%         % $\mc{R}(z_\phi, z_\psi, \nu) \triangleq \lambda||\mf{H}^\phi_\nu(z_\phi) - \mf{H}^\phi_{\nu_0}(z_\phi)||^2_2 + \lambda||\mf{H}^\psi_\nu(z_\psi, \mf{H}^\phi_\nu(z_\phi)) - \mf{H}^\psi_{\nu_0}(z_\psi, \mf{H}^\phi_{\nu_0}(z_\phi))||^2_2$
        
%         % $\mc{L}(\nu,\tilde{\mc{D}}) = \bE_{\substack{z_\phi \sim p_z(\cdot) \\ z_\psi \sim p_z(\cdot)}}[\frac{1}{m} \sum\limits_{\tilde{\mc{D}}}(r + \max\limits_{a' \in \mc{A}}     \hat{Q}^\star_{z_\phi,z_\psi}(s',a') + \eta_\phi^Tz_\phi + \eta_\psi^Tz_\psi - \hat{Q}^\star_{z_\phi,z_\psi}(s,a))^2 +  \mc{R}(z_\phi, z_\psi, \nu)]$
        
%         $\nu \leftarrow \nu - \alpha \nabla_\nu \mc{L}(\nu,\tilde{\mc{D}})$
%     }
% }

% \end{algorithm}
